A Hierarchical Block Distance Model for Ultra Low-Dimensional Graph Representations

Graph Representation Learning (GRL) has become central for characterizing structures of complex networks and performing tasks such as link prediction, node classification, network reconstruction, and community detection. Whereas numerous generative GRL models have been proposed, many approaches have prohibitive computational requirements hampering large-scale network analysis, fewer are able to explicitly account for structure emerging at multiple scales, and only a few explicitly respect important network properties such as homophily and transitivity. This paper proposes a novel scalable graph representation learning method named the Hierarchical Block Distance Model (HBDM). The HBDM imposes a multiscale block structure akin to stochastic block modeling (SBM) and accounts for homophily and transitivity by accurately approximating the latent distance model (LDM) throughout the inferred hierarchy. The HBDM naturally accommodates unipartite, directed, and bipartite networks whereas the hierarchy is designed to ensure linearithmic time and space complexity enabling the analysis of very large-scale networks. We evaluate the performance of the HBDM on massive networks consisting of millions of nodes. Importantly, we find that the proposed HBDM framework significantly outperforms recent scalable approaches in all considered downstream tasks. Surprisingly, we observe superior performance even imposing ultra-low two-dimensional embeddings facilitating accurate direct and hierarchical-aware network visualization and interpretation.

==> 0-abstract.tex <==
\begin{abstract}
Graph Representation Learning (GRL) has become central for characterizing structures of complex networks and performing tasks such as link prediction, node classification, network reconstruction, and community detection. Whereas numerous generative GRL models have been proposed, many approaches have prohibitive computational requirements hampering large-scale network analysis, fewer are able to explicitly account for structure emerging at multiple scales, and only a few explicitly respect important network properties such as homophily and transitivity. This paper proposes a novel scalable graph representation learning method named the Hierarchical Block Distance Model (HBDM). The HBDM imposes a multiscale block structure akin to stochastic block modeling (SBM) and accounts for homophily and transitivity by accurately approximating the latent distance model (LDM) throughout the inferred hierarchy. The HBDM naturally accommodates unipartite, directed, and bipartite networks whereas the hierarchy is designed to ensure linearithmic time and space complexity enabling the analysis of very large-scale networks. We evaluate the performance of the HBDM on massive networks consisting of millions of nodes. Importantly, we find that the proposed HBDM framework significantly outperforms recent scalable approaches in all considered downstream tasks. Surprisingly, we observe superior performance even imposing ultra-low two-dimensional embeddings facilitating accurate direct and hierarchical-aware network visualization and interpretation.
%Graph Representation Learning (GRL) has become a prominent approach in understanding the underlying intrinsic structures of complex networks and performing various tasks over graph-structured data. Recently, various generative methods have been developed for the analysis of social networks. However, very few approaches learn latent embeddings of nodes explicitly respecting networks’ homophily and transitivity properties, such as the prominent Latent Distance Model (LDM). Many approaches also have problems extracting embeddings for large-scale networks due to their computational requirements, and even fewer methods allow for learning hierarchical representations. This paper proposes a novel graph representation learning method named the Hierarchical Block Distance Model (HBDM). It extracts node embeddings imposing a multiscale block-structure that accounts for homophily and transitivity properties across the levels of the inferred hierarchy. Notably, the HBDM naturally accommodates unipartite, directed, and bipartite networks whereas the hierarchy is designed to ensure linearithmic time and space complexity enabling the analysis of very large-scale networks. We evaluate the performance of our approach on massive networks consisting of millions of nodes. Our HBDM framework  significantly outperforming recent scalable approaches in downstream tasks providing superior performance even using ultra low-dimensional embeddings at the same time facilitating direct and hierarchical-aware network visualization and interpretation.
%Graph Representation Learning (GRL) has become a prominent approach in understanding the underlying intrinsic structures of complex networks and performing various tasks over graph-structured data. Recently, various generative methods have been developed for the analysis of social networks. However, very few approaches learn latent embeddings of nodes explicitly respecting networks’ homophily and transitivity properties, such as the prominent Latent Distance Model (LDM). Many approaches also have problems extracting embeddings for large-scale networks due to their computational requirements, and even fewer methods allow for learning hierarchical representations. This paper proposes a novel graph representation learning method named the Hierarchical Block Distance Model (HBDM). It extracts node embeddings in a multiscale block-structured way while naturally expressing homophily and transitivity properties in all levels of the hierarchical structure. Notably, our proposed model is characterized by a linearithmic time and space complexity in terms of network size. Thereby it enables the analysis of very large-scale networks, combining LDM with a tailored clustering procedure responsible for imposing the multiscale hierarchical structure. We evaluate the performance of our approach on massive networks consisting of millions of nodes. Our HBDM framework, shows high performance with ultra low-dimensional embeddings in downstream tasks and facilitates direct and hierarchical-aware network visualization and interpretation while significantly outperforming recent scalable approaches.

%Graph Representation Learning (GRL) has become a prominent approach in understanding the underlying intrinsic structures of complex networks and performing various tasks over graph-structured data. In recent years, various generative methods have been developed for the analysis of social networks. However, very few approaches learn latent embeddings of nodes explicitly respecting networks' homophily and transitivity properties, such as the prominent Latent Distance Model (LDM) models. Many approaches also have concerns in extracting embeddings for large-scale networks due to their computational requirements, and even very few methods allow us to learn hierarchical representations. This paper proposes a novel graph representation learning method named the Hierarchical Block Distance Model (HBDM). It extracts node embeddings in a multiscale block-structured way while naturally expressing homophily and transitivity properties in all levels of the hierarchical structure. Notably, our proposed model is characterized by a linearithmic time and space complexity in terms of the number of nodes in the network, $\mathcal{O}(N\log{N})$. Therefore, allows for the analysis of very large-scale networks, combining LDM with a tailored clustering procedure responsible for imposing the multiscale hierarchical structure.We evaluate the performance of our approach on massive networks consisting of millions of nodes. We show that our approach significantly outperforms the recent scalable approaches in node classification and link prediction tasks. Although baseline methods require much higher dimension sizes to compete against the proposed method, we utilize tiny embedding sizes of two and three. The proposed method shows high performance with ultra low-dimensional embeddings in downstream tasks and facilitates direct and hierarchical-aware network visualization and interpretation.
\end{abstract}

\noindent%
{\it Keywords:} graph representation learning, link prediction, low-dimensional embeddings, latent-space, networks, large-scale

==> 3-related_work.tex <==
\subsection{Related Work}
%In recent years, we have witnessed a tremendous increase in the number of GRL methods. The leading initial works are the random walk-based methods \cite{deepwalk-perozzi14, node2vec-kdd16, line, expon_fam_emb, biasedwalk}, which generate fixed-length node sequences by following a strategy and leverages the Skip-Gram algorithm \cite{MSCC+13} to learn the node representations. Another prominent class of techniques is the matrix factorization-based algorithms \cite{cao2015grarep, HOPE-kdd16, GRL-survey-ieeebigdata20}. They extract the embedding vectors by decomposing a designed feature matrix. The neural networks are undoubtedly one of the most outstanding models, and many models \cite{GRL-survey-ieeebigdata20, SDNE-kdd16, GRL-survey-ieeebigdata20, SDAE_aaai16_shaosheng, gcn_jclr17_kipf, graphsage_hamilton} have been proposed for graph-structured data that allow to incorporate the node attributes with the network structure when learning the embeddings . Although these approaches are quite effective in downstream tasks, they require a high computational burden, making them inapplicable for large networks. Therefore, the recent works \cite{louvainNE-wsdm20, prone-ijai19} capitalize on the computational challenges emerging for large networks by either incorporating approximation techniques for the existing models \cite{netsmf-www2019} or developing novel approaches based on hashing schemes \cite{YRLC19, randne-icdm18}. Our approach relates to current efforts for scaling GRL for the analysis of large networks.

In recent years, we have witnessed a tremendous increase in the number of GRL methods. The leading initial works are the random walk-based methods \cite{deepwalk-perozzi14, node2vec-kdd16, line, expon_fam_emb, biasedwalk}, leveraging the Skip-Gram algorithm \cite{MSCC+13} to learn the node representations. Matrix factorization-based algorithms \cite{cao2015grarep, GRL-survey-ieeebigdata20} are also prominent, extracting the embedding vectors by decomposing a designed feature matrix. Neural network models \cite{GRL-survey-ieeebigdata20, GRL-survey-ieeebigdata20, graphsage_hamilton} have been proposed for graph-structured data, returning outstanding performance by combining node attributes with the network structure for learning the embeddings. Recent works \cite{louvainNE-wsdm20, prone-ijai19} capitalize on the computational challenges of the previous methods, emerging for large networks, by either incorporating approximation techniques for the existing models \cite{netsmf-www2019} or by fast hashing schemes \cite{randne-icdm18}. Our approach relates to current efforts for scaling GRL for the analysis of large networks.


Prior works, have endowed the \textsc{LDM} with a clustering model enforcing a Gaussian Mixture Model as a prior over the latent variables, defining the Latent Position Clustering Model (\textsc{LPCM}) \cite{LPC,KRIVITSKY2009204}. The \textsc{LPCM} framework, defines block structures accounting for both homophily and transitivity but do not provide hierarchical structures, as the proposed \textsc{HBDM}. In addition, \textsc{LPCM} does not scale for large networks. A possibility for obtaining a scalable homophilic block representation is through a two-stage optimization procedure via the case-control \textsc{LDM} \cite{case_control}. Such a procedure would firstly optimizes the \textsc{LDM} and then imposes a clustering procedure, as a post-processing step. Notably, such an approach does not yield a natural block representation of network structure as the presently developed \textsc{HBDM}. Meaning that the post-processing clustering, does not utilize information from the imposed hierarchical cluster structure during the construction of the latent space which is useful when estimating the latent positions nor exploits how the hierarchical structure admits scalable inference.

%Essentially, Eq. \eqref{eq:log_likel_lsm} can be separated in two populations of cases (edges) and controls (non-edges) and regard the quantity $p_0$ as a total population statistic, with the authors proposing an unbiased estimation via stratified sampling over the shortest path information between nodes as a "closeness" metric in order to define the importance of each the strata. 
%While the overall complexity of the case-control model can scale the analysis of \textsc{LDM}s to massive networks creating the All-Pairs Shortest Paths matrix that is required to perform the proposed stratified sampling over non-links, is not possible for large networks, both in terms of time and space complexity ($>\mathcal{O}(N^2)$) and the authors did not consider networks larger than $N=2716$ nodes. In the supplementary material, we therefore examine a scalable version of the case-control approach. In order to scale the case-control model to the order of millions of nodes as presently considered we exchanged the stratified sampling with a uniform sampling procedure which as argued by the authors may not be the best estimator. 
%Nevertheless, we discovered that the case-control model has a surprising link-predictive performance equivalent to our proposed \textsc{HBDM} even though it visits a very limited number of non-edge pairs of the network. 
 %We conclude that also the case-control approach can be used to successfully scale the \textsc{LDM}s. Notably, the case-control approach does not yield a hierarchical representation of network structure as the presently developed \textsc{HBDM}. However, the developed hierarchical clustering procedure can be used as a post-processing step to extract hierarchical representations from the learned embeddings.

==> 6-conclusion.tex <==
\section{Conclusion}\label{limitations}
 
%Presently, the main bottleneck of the \textsc{HBDM} approach is the computations required for the Euclidean k-means procedure proposed. Future work should investigate how the presented auxiliary function optimization procedure can be improved by exploring existing procedures scaling conventional squared Euclidean k-means by avoiding unnecessary distance calculations \cite{elkan2003using} or by use of binary space partitioning trees \cite{pettinger2010space}. Such improved scaling would admit utilization of non-binary splits beyond the root node improving the accuracy of the hierarchical approximation. 


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

